Conformal Set-based Human-AI Complementarity with Multiple Experts

Decision support systems are designed to assist human experts in classification tasks by providing conformal prediction sets derived from a pre-trained model. This human-AI collaboration has demonstrated enhanced classification performance compared to using either the model or the expert independently. In this study, we focus on the selection of instance-specific experts from a pool of multiple human experts, contrasting it with existing research that typically focuses on single-expert scenarios. We characterize the conditions under which multiple experts can benefit from the conformal sets. With the insight that only certain experts may be relevant for each instance, we explore the problem of subset selection and introduce a greedy algorithm that utilizes conformal sets to identify the subset of expert predictions that will be used in classifying an instance. This approach is shown to yield better performance compared to naive methods for human subset selection. Based on real expert predictions from the CIFAR-10H and ImageNet-16H datasets, our simulation study indicates that our proposed greedy algorithm achieves near-optimal subsets, resulting in improved classification performance among multiple experts.

==> 3.old_framework_prelim.tex <==
% PRELIM: 5/10
\section{Preliminary}
\label{3.framework_prelim}




\subsection{Problem Formulation}

% sources: EPCP 



The target of multi-class classification is to predict the corresponding label $y \in \mathcal{Y} = \{1,...,n\}$ from the feature vector $x \in X$. The random variables $(x, y)$ follows an unknown distribution. In human-AI systems, an automated decision support $C:\mathcal{X} \rightarrow 2^\mathcal{Y}$, predicts a set of potential labels $C(x) \subseteq\mathcal{Y}$. At the same time, a human expert labeler is accessible, represented by the function $h:\mathcal{X}\to\mathcal{Y}$. %gives a final prediction $h(x)\in C(x)$ based on the set $C(x)$. 
Here the system is usually established based on a pre-trained classifier $\hat{f}: \mathcal{X}\rightarrow[0,1]^{|\mathcal{Y}|}$, where $\hat{f}(x)$ is the normalized probability vector and $C(x)$ is determined based on the outputs scores $f(x)$. The system intends to help human experts by narrowing down the scope of prediction. The objective of this work is to create a framework for performing inference by integrating multiple human experts and the system $C$. To be specific, suppose there are $m$ human experts, and the $i$th  predicts label $\hat{y}_i$ for the instance $x$. From the multiple human predictions $\{\hat{y}_i\}_{i=0}^m$, we intend to derive a framework to come up with the final prediction $\hat{y}$. We expect our designed system to benefit from the collaborative decisions of multiple human experts in a way that:

\begin{center}
$P(\hat{y}=y;C) \geq P(\hat{y}_i=y;C) \geq P(\hat{y}_i=y;\mathcal{Y})$ for $i\in \{0,1,...,m\}$
\end{center}
where %$\hat{Y}$ represents the collaborative prediction from the multiple human experts, $Y_i$ represents the prediction of the single expert $i$, and 
$P(\hat{y};C)$ indicates the probability of the collaborative decisions $\hat{y}$ (based on the system $C$) is the same as the label $y$.




\subsection{Confusion Matrix of Humans}
% For an instance $x$, each human from a team of $n$ humans provides a hard label $h_i(x)$ where $h_i(x)$ can be any of the k possible labels. Collection of human labels for an instance $x$ is denoted as $h(x) = \{h_1(x), h_2(x), \cdots, h_n(x)\}$. 
Given an instance and label pair $(x,y)$ and a human label $h(x)$, let $\psi_{ij}:=P(h(x)=i\mid y=j)$ denote the conditional probability that the human labeler predicts label $i$ given that the true label is $j$. Then the $n\times n$ confusion matrix for the human is defined as  $\psi=(\psi_{ij})^n_{i,j=1}$. In this work, we estimate the confusion matrix by the maximum likelihood method as in  \citet{Straitouri2022ImprovingEP}.

% a human expert $i$ predicts a label $\hat{y}$ based on the instance $x$. L
% {\color{blue} Read comment by HP}
% {\color{red}
% I am confused. I don't know the reason to introduce $H$ and ${\Psi}_{qr}$ here. Did you use these notations later? Please revise this part, pay attention to the logic, and delete this part if there is no need to introduce it.}

 In addition to the confusion matrix, for an instance $x_i$, %each human from a team of $n$ humans provides a hard label $h_i(x)$ where $h_i(x)$ can be any of the k possible labels. Collection of human labels for an instance $x$ is denoted as $h(x) = \{h_1(x), h_2(x), \cdots, h_n(x)\}$. 
we assume access to $H(x_i) = (H_j(x_i))_{j=1}^n$ which is a vector that collects the predictions of human labelers on the instance $x_i$, where $H_k(x_i)$ denotes the total number of human labelers who predicted class $k$. Given an instance $x_i$ and experts predictions $H$, we can calculate the empirical distribution of human predictions by ${\Psi}_{ij} = P(h(x_i)=j) = H_j(x_i) / \sum_{k=1}^{n} H_k (x_i)$, $1 \leq j \leq n$. Then the human empirical distribution for the test data is denoted by $\Psi = (\Psi_{ij})$ where $i=1,\hdots, T$ and $j=1,\hdots, n$. Our approach utilizes the distribution of expert predictions $\Psi$ to simulate initial human predictions. This step is necessary during inference of proposed framework\footnote{The approach by \citet{Straitouri2022ImprovingEP} lacks a clear inference stage, as their inference stage utilizes ground truth labels for the test data, which is unrealistic in practical scenarios.}.  We combine human predictions with the predicted conformal sets instead of merging predictions from a single human with class-wise model probabilities as in \cite{Kerrigan2021CombiningHP,Singh2023OnSS}. The upper right part of Figure \ref{fig:comb_framework} demonstrates our proposed inference.
 



%From $h(x)$, we calculate the confusion, which we denote as $\psi$. Mathematically, it represents the probability that a human assigns label $i$ when the true label is $j$, i.e. $\psi_{ij} = p(\hat{Y}_i = i| y(x) = j)$. 
% , defined as:

% \begin{center}
% $\psi_{ij} = \frac{{\sum_{x \in X} I(h (x) = i \: \land \: y(x) = j)}}{{\sum_{x \in X} I(y(x) = j)}}$ 
% \end{center}

% where $I(\cdot)$ is an indicator function. 

% Several factors contribute to the performance of the combined model: the accuracy of the pretrained model $M$, the confusion matrix of the humans, the number of humans in the ensemble, and the framework to decide the final prediction based on the ensemble of experts.

%For simplicity, we assume that each human has the same confusion matrix. A straightforward method to estimate the confusion matrix involves maximum likelihood estimation.

% {\color{red} Read comment by HP}
% {\color{blue}
% ！！Unclear, what is different from our methods in terms of the confusion matrix? You should be specific in math. to illustrate the difference.！！}













% Discuss here about conformal prediction
% sources: Class-conditional conformal prediction, EPCP
\subsection{Conformal Prediction}

Given a dataset and a test sample $(x_{test}, y_{test})$, the goal of conformal prediction is to construct a prediction set $C(x_{test})$ based on the dataset such that it satisfies the marginal coverage at a user-specified level $\alpha \in [0,1]$ in the sense that 
\begin{equation}
    \mathbb{P}(y_{test} \in {C} (x_{test})) \geq 1- \alpha.
\end{equation}

 The constructed set $C(x_{test})$ can be established based on any pre-trained classifier $\hat{f}$ without relying on any distributional assumptions about the data \citep{Vovk2005AlgorithmicLI}.

Given a pre-trained classifier $\hat{f}$ and a dataset $D_{\text{cal}} = (x_i, y_i)_{i=1}^l$ with independent and identically distributed sample.
To construct a conformal prediction, 
we calculate the conformal score $s:\mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}$ by $s(x_i, y_i) = 1 - \hat{f}_{y_i}(x_i)$ on each sample, where $\hat{f}_{y_i}(x_i) $ denotes predicted probability for label $y_i$ on $x_i$. A lower conformal score $s(x_i, y_i)$ means better agreement between the input $x_i$ and the label $y_i$. While a conformal score is close to one implies the pre-trained classifier is significantly incorrect on $x_i$. Let $\hat{q}_{\alpha}$ be the empirical $\lceil (l+1)(1-\alpha) \rceil$-th quantile of the conformal scores $s(x_1, y_1), \ldots, s(x_l, y_l)$. Then conformal prediction set $C(x_{test})$ is constructed by
$C(x_{test}) = \{y : s(x_{test}, y) \leq \hat{q}_\alpha\}$. One can show that conditioned on the calibration set $D_{\text{cal}}$, the probability of the true label $y_{test}$ belonging to the subset $C(x_{test})$ is guaranteed larger than $1-\alpha$ \cite{Angelopoulos2021AGI}. 
% \vspace{-1em}
%{\color{red} Please cite the original paper giving the proof of the guarantee. It should be a paper from Cand\'es.}


% with high confidence, provided that the size $l$ of the calibration set is sufficiently large. 




%Notably, the coverage probability is a random quantity with a distribution described by the following proposition 
%(see Appendix A.5 in Hulsman (2022) for the proof).





==> 3.old_framework_proposed.tex <==
% Proposed Framework: 5/10
\section{Proposed Framework}
\label{3.framework_proposed}
% \vspace{-1em}

In this section, we propose the conformal multi-expert approach for combining multiple human predictions with the pre-trained-model-based conformal sets. We also propose an algorithm that estimates the optimal number of human experts to be utilized during inference. The intuition is that with a huge number of experts, the pre-trained model may not be necessary and the expert team could already achieve success prediction on their own. 
% \vspace{-1em}

\subsection{Combining Conformal Sets and Human Predictions During Inference}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=14cm]{images/topic_proposed/proposed_comb.jpg}
%   \caption{Visualization of the inference procedure of simulating multiple humans from $\Psi$ and combining the expert prediction and the conformal set. On the left, we utilize the expert predictions on the estimation and calibration data to generate the confusion matrix. }
%   \label{fig:comb_framework}
%   \vspace{-2em}
% \end{figure}

In the human-AI system, the conformal set prediction is combined with the human experts' prediction. We extend the framework from a single expert to  multiple simulated human predictions.

% {\color{blue} Comment by HP }
% {\color{red}
% ???It is unclear to me. $\psi_{syn}$ is supposed to be an entry of the confusion matrix, and why it is determined by $h_{syn}$ here ????}

For a test instance $x_i$, the conformal predictor utilizes the score from the pre-trained machine learning classifier to predict a conformal set. We let the vector $(c_j)_{j=1}^n$ to denote the conformal set, where $c_j = 1$ if class $j$ is in the conformal set, and $c_j = 0$ otherwise.  Then the human experts decisions are simulated in the following way. Firstly an initial human label $\kappa$ is drawn following the distribution $\Psi_{i} = (\Psi_{ij})_{j=1}^{n}$. %the test expert distribution for instance $x_i$.
 Then the $\kappa$th row of the confusion matrix $\psi_{\kappa} = (\psi_{\kappa,j})_{j=1}^n$ is used to weight the elements within the conformal set. Specifically, we normalize the vector $(c_j \times \psi_{\kappa,j})_{j=1}^n$ such that it is a probability vector with entries sum up to 1. By sampling from the multinomial distribution defined by the normalized probability vector, we obtain the final prediction of a single expert. 
 
% This procedure is visualized in the lower right of Figure \ref{fig:comb_framework}.
% Consequently, $\psi_{syn}$ is employed to weigh the conformal sets, thus creating a categorical distribution for the elements within the conformal set to incorporate human preference.


% Given the labels of $n$ humans, we create an expert class distribution, denoted as $\Psi$, with which we can also generate the confusion matrix $\psi$. Calculating the expert distribution can be done by normalizing predictions for each instance across all classes. 
% Note that we can infinitely sample predictions from this distribution.

% {\color{blue}
% !!!There is no pre-context in the following two paragraph. What brought you to introduce the two cases in the following? I am very confused about why it suddenly comes two paragraphs without any pre-context. Pay attention to the COHERENCE of the paper.!!!
% }


% Second Case: Alternatively, one might argue for directly using the test expert distribution $\Psi_i = [\Psi_{i0}, \Psi_{i1}, \ldots, \Psi_{in}]$ to weigh the conformal sets. This approach involves forming a multinomial distribution defined by $[c_0 \cdot \Psi_{i0}, c_1 \cdot \Psi_{i1}, \ldots, c_n \cdot \Psi_{in}]$ and generating a single sample as the final prediction from this distribution. However, we will demonstrate that sampling a human label $h_{syn}$ and using this label to derive a class distribution from the mean confusion matrix provides superior results. 

%Theorem: Proof is in the appendix.
%\textbf{Remarks:} 

% {\color{blue}
% !!The same issues of COHERENCE. It suddenly appears a subtitle of ``Removing the search for optimal $\alpha$" without any pre-context and explanation. It is unfriendly to readers.
% !!
% }



% Note that we could also utilize real predictions from multiple experts given that we have a dataset where we know what label each individual expert gave. But in some datasets, only a final tally of predictions for each class is given. On the other hand, real multiple experts data gives us deterministic prediction from any single expert. 
%Actually baka pwede sa NIH Dataset.













% MAKE PICTURES FOR THESE APPROACHES
\subsection{Extending to Multiple Experts}

% What is this framework all about? What is the general intuition? Why do we do this? What frameworks do we devise? What is the intuition with these devised frameworks? 
We extend the framework to incorporate simulated predictions from multiple humans. To the best of our knowledge, this is the first work to understand whether multi-expert collaboration can achieve desirable accuracy or success probability even when the options are narrowed down. 

% Reducing the set of options simplifies the cognitive workload for the experts. 
% From intuition, it seems to make sense that multiple experts are better than a single expert. Moreover, judgments from multiple experts picking a choice from the conformal set can result in an improved final prediction.  
%We propose an approach that favors that majority of expert predictions (called the mode) and propose other approaches which can be thought of as combining multiple human predictions to redefine the distribution of the labels in predicted conformal set from the pre-trained classifier.



% Efficiency of the mode etc
% TODO WHAT IF BIMODAL CASE?
A straightforward approach to integrating multiple experts' predictions is to choose the majority prediction as the final prediction. In the experimental results, we refer to this as the \textbf{mode approach}. 

% Another approach is \textbf{sampling-based}. The idea is to calculate class weights based on the simulated predictions to indicate how likely a test instance is categorized as that class. 

% Given a test instance $x_i$ and $m$ simulated predictions from the empirical distribution of expert labels $\Psi_{i} = (\Psi_{ij})_{j=1}^{n}$.
% Let $e_{i,j}$ denote the number of simulated human predictions for class $j$ and let weights $w_{i,j} = e_{i,j}/m$. Recall $\psi_k = (\psi_{k,j})_{j=1}^n$ denotes the $k$th row of the confusion matrix. Then the final conformal set weights $\tau_i$ for a test instance $x_i$ is calculated as $\tau_i = (\tau_{i,j})_{j=1}^n = \sum_{j=1}^{n} w_{i,j} \cdot \psi_j$. 
% In addition, there is  \textbf{empirical distribution-based approach}. For a single test instance $x_i$, the weights $w_{i,h}$ for each class are exactly the values from the empirical distribution of expert prediction $\Psi_i = (\Psi_{i,h})_{h=1}^n$. The final conformal set weights are calculated as $\tau_i = (\tau_{i,j})_{j=1}^n = \sum_{h=1}^{n} \Psi_{i,h} \cdot \psi_{h}$. 








% What is meant by optimal number for a given task? Is there a factual reference to this? What is this framework all about? Why do we need this? % Add factual reference

\textbf{Determining the size of the multi-expert team for inference.} Increasing the number of human experts incurs higher resource costs. Additionally, a large team of experts may render a pre-trained model unnecessary, as the team alone could perform classification effectively. Therefore, we aim to determine the optimal number of experts, $\hat{m}$, for a given task. Using a hold-out estimation dataset, we develop an algorithm to find $\hat{m}$, the maximum number of experts that should be utilized during inference to ensure they still benefit from the pre-trained model. Algorithm \ref{algo:optimal_m} outlines this framework. During inference, decision-makers can select the number of experts from the range $[1, \hat{m}]$. Exceeding $\hat{m}$ may not provide additional benefits, and a larger team might perform better independently. For a detailed description of the algorithm, see Section \ref{algo_description} of the Appendix. % Conversely, a small number of experts might not achieve the best success probability, which could maximize the utility of the pre-trained model that generates the narrowed set of options for the experts. 



Based on \cite{Singh2023OnSS}, we propose a method to calculate the subset of humans in our combination approach  for conformal multi-expert. A subset of the optimal m experts will be assigned to each sample.


% Why should we remove alpha? Is this valid?
\textbf{Removing the search for optimal $\alpha$}. \citet{Straitouri2022ImprovingEP} aims to maximize the empirical success probability of the expert during inference by optimizing the conformal predictor's $\alpha$ during the estimation stage with hold-out data. In conformal prediction, $\alpha$ denotes the miscoverage risk, the maximum allowable probability that the true label is excluded from the predicted conformal set. Figure \ref{fig:optimal_alpha_cifar} shows that selecting a small $\alpha$ is preferable, as it increases the conformal set's coverage and correlates with higher empirical success probability. Therefore, in our proposed framework, we fix $\alpha$ at a low value rather than calculating the optimal $\alpha$, and use the estimation data to determine $\hat{m}$.


% Two column style for the algorithm % on the left you show content, on the right, you may prepare a picture to demonstrate the algorithm

\begin{figure}[h!]
    \centering
    \begin{minipage}{0.49\textwidth}
        \begin{algorithm}[H]
        \caption{Finding the suggested maximum number of experts $\hat{m}$}
        \label{algo:optimal_m}
        \begin{algorithmic}[1]
        \REQUIRE $\hat{f}$, $D_{\text{est}}$, $D_{\text{cal}}$, $\delta$, $\zeta$
        \STATE \textbf{Initialize:} $M = \{\}$, $\hat{m} \gets 1$, $t \gets 0$
        \FOR{$i \in 1, \dots, \zeta$}
            %\STATE $\alpha \gets 1 - \frac{i}{m+1}$
            \STATE $M \gets M \cup i$
        \ENDFOR
        \FOR{$m \in M$}
            \STATE $\hat{\Phi}_E \gets \text{GET\_ACC\_EXPERTS}(M)$
            \STATE $\hat{\Phi}_\alpha \gets \text{ESTIMATE}(m, \alpha, \delta, D_{\text{est}}, D_{\text{cal}}, \hat{f})$
            \IF{$t \geq \hat{\Phi}_\alpha \geq \hat{\Phi}_E$} % - \epsilon_{\alpha,\delta}/m$
                \STATE $t \gets \hat{\Phi}_\alpha$ %- \epsilon_{\alpha,\delta}/m
                \STATE $\hat{m} \gets m$
            \ENDIF
        \ENDFOR
        \RETURN $\hat{m}$
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}
    \hfill
    \begin{minipage}{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/topic_proposed/optimal_m_Preresnet.jpg}
        \caption{Using the hold-out estimation data on the CIFAR-10H dataset with size of 1000, we calculate $\hat{m}=3$ using Algorithm \ref{algo:optimal_m} when using a pre-trained PreResNet Model. This informs decision-makers that the suggested number of experts during inference should fall on $[1,3]$.}
        \label{fig:find_m_preresnet_sample}
    \end{minipage}
\end{figure}

















==> 4.old_experiments__setup.tex <==
\section{Experimental Results}
\label{4.experimental_setup}







\subsection{Dataset Description}

We applied the framework to two real-world datasets to assess its practical utility. These datasets were selected as benchmarks for integrating the conformal prediction framework with multiple experts.

% What is this dataset all about? Why did you use this dataset?
\textbf{CIFAR-10H Dataset} \cite{Peterson2019HumanUM}. This dataset is a collection of 10,000 natural images taken from the test set of the standard CIFAR-10 \cite{Krizhevsky2009LearningML}.  Prior works \citep{Kerrigan2021CombiningHP, Straitouri2022ImprovingEP, Singh2023OnSS}, which serve as our baselines, utilized this dataset. We evaluate our conformal multi-expert framework against these established benchmarks.

% What is this dataset all about? Why did you use this dataset?
\textbf{ImageNet-16H Dataset} \cite{Steyvers2022BayesianMO}. The images and categories in this dataset are based on a subset of the ImageNet Large Scale Visual Recognition Challenge (ILSRVR) 2012 database \cite{Russakovsky2014ImageNetLS}. Each image can be categorized into one of the 16 classes, where each one has separate human annotations. Overall, there are 1200 unique images with equal division among several classes.  To make the annotation for humans and classifiers more challenging, images are distorted via spatial frequency phase noise of $\omega$ = 80. This dataset is utilized in this work to further understand how the conformal-based multi-expert framework works in the setting where there are many classes and limited calibration data.
\vspace{-1em}
% different levels $\omega$ = {80, 95, 110, 125}
    
    % \item HateSpeech. This dataset consists of around 25k labeled tweets based on [cite]. There are three classes which are the following: hate speech, offensive but not hate speech, or neither offensive nor hate speech. The annotator is random.
    % \item COMPASS Dataset. This dataset consists of two classes. It has a separate human annotator.
    
% \textbf{NIH Chest X-ray} \cite{Majkowska2019ChestRI}. Collected by the NIH Clinical Center, this dataset consists of the annotations of radiologists from the ChestX-ray8 dataset \cite{Wang2017ChestXRay8HC}. Specifically, they annotated the four radiographic findings on a subset of 4,374 chest X-ray images. It consists of around 4k samples where each sample can be categorized in one of two classes.


    


\subsection{Experimental Setup}

% What is the description of the dataset, pretrained models used?

For the CIFAR-10H dataset, we employ five widely-used deep learning models: DenseNet, ResNet110, PreResNet-110, and two less accurate models, CNN \cite{Singh2023OnSS} and a low accuracy model \cite{Kerrigan2021CombiningHP}. In the empirical evaluation, we adopt a data split strategy of 80\% for testing, 10\% for calibration, and the remaining 10\% for estimation purposes. For the ImageNet-16H dataset, we train our own model and assess various approaches using two data split configurations: $v1$ (15\% train, 5\% validation, 80\% test) and $v2$ (30\% train, 10\% validation, 60\% test). The test data is further divided into test (60\%), calibration (28\%), and estimation (12\%) subsets. Human prediction tallies $H$ on non-test samples are used to estimate the confusion matrix $\psi$ (see Figure \ref{fig:comb_framework}, left). For classification tasks, we measure test data accuracy (empirical success probability). For frameworks using conformal sets, we calculate average set sizes and class-conditional coverage. We compare our results with the following relevant baselines: combination approach with MAP temperature scaling \cite{Kerrigan2021CombiningHP}, Mode Approach (Multi-expert) from \cite{Singh2023OnSS} \footnote{Note that this work presents multiple approaches for human-AI combination, but we select the one with the highest accuracy on the test data.}, and conformal-based single expert approach \cite{Straitouri2022ImprovingEP}. These baselines are chosen because they align with our methodology, focusing on leveraging pre-trained classifier outputs and combining them with simulated expert predictions during inference.
\vspace{-1em}
% Average set size reflects the uncertainty of the pretrained model, while class coverage indicates the reliability of the predicted conformal sets.

% Remove this for now.
% For the NIH Chest X-ray dataset, we can only conduct experiments up to a maximum of two real human experts due to data insufficiency. We perform experiments with 4 pairs of radiologists where each pair of radiologist annotated around 800 common images. For each run, we partition the data into 40\% train data, 10\% validation data, and 50\% test data. The models are trained for 50 epochs using Adam optimizer with a learning rate of 1e10-3, weight decay of 5e10-4, and a batch size of 64. The experiments are repeated 10 times with varying seeds.

% --What are the evaluation metrics used? Why use these? Are there evaluation metrics used for conformal prediction? How did you evaluate the dataset with more classes?
% --What are the baselines we use? % Why use these baselines and what is the intuition??




==> 4.old_experiments_cifar.tex <==













\subsection{Experimental Results}
\label{4.experimental_res}

\subsubsection{CIFAR-10H}




% How does our framework compare with the baselines? What can we observe from the results? Why is this the case?
\textbf{Comparison with Human-AI Combination Approaches.}
In Table \ref{tab:cifar10h_results_baselines}, we compare the empirical success probability on the test data of our proposed conformal-based multi-expert mode-based framework to existing approaches that combine pre-trained classifier outputs with human predictions. The results demonstrate that multi-expert collaboration enhances empirical success probability. Even with a reduced set of options for the humans, our framework outperforms previous baselines where humans had the full set of labels to choose from. Notably, with the less accurate pre-trained CNN classifier, existing approaches fail to surpass the performance of a single human. 
%Additionally, the framework by \citet{Straitouri2022ImprovingEP}, which uses the ground truth label during inference, also does not achieve a higher empirical success probability.



% Include Expert Team? How about Classifier Team?
\begin{table}[ht!]
    \setlength{\tabcolsep}{1.15pt}
    \small  
    \centering
    \vspace{-1em}
    \caption{Empirical success probabilities achieved by our conformal mode-based multi-expert approach using five neural network-based pre-trained classifiers and five multiple experts ($m=5$) in comparison with previous baselines during testing on the CIFAR-10H dataset. The calibration and estimation sets each have a size of 1,000. The final row displays the official framework from \citet{Straitouri2022ImprovingEP}, which uses the test labels during inference.}
    \vspace{1em}
    \begin{tabular}{|l|c|c|c|c|c|}
    \hline
        Model Name & Densenet &	Resnet & Preresnet & CNN & Low Acc  \\
        \hline 
        Pre-trained Model Alone & 96.29 $\pm$
0.09 & 92.70 $\pm$ 0.20 & 94.41 $\pm$
0.12 & 51.00 $\pm$ 0.54 & 87.09 $\pm$ 0.30   \\
        Single Human Alone	& 95.16 $\pm$ 0.24 & 95.24 $\pm$ 0.26 & 95.27 $\pm$ 0.21 & 94.86 $\pm$ 0.18 & 95.16 $\pm$ 0.14  \\
        \hline
        \citet{Kerrigan2021CombiningHP} (MAP temp. scaling)  & 97.81 $\pm$ 0.25 & 97.22
$\pm$ 0.40 & 97.56 $\pm$ 0.36 & 93.92
 $\pm$ 0.54 & 96.39 $\pm$ 0.32         \\
        \citet{Singh2023OnSS} (Mode - mult. experts) & 97.93 $\pm$ 0.13 & 97.23 $\pm$
0.19 & 97.48 $\pm$ 0.16 & 92.51 $\pm$
0.20 & 96.39 $\pm$ 0.25   \\ 
        \citet{Straitouri2022ImprovingEP} (single expert)  & 97.70
$\pm$ 0.09 & 96.63 $\pm$ 0.13 & 97.05 $\pm$ 0.18 & 89.76 $\pm$ 0.21 & 95.01 $\pm$ 0.33 \\
        Conformal Multi-expert & \textbf{98.44
$\pm$ 0.23} & \textbf{98.03 $\pm$ 0.23} & \textbf{98.06 $\pm$ 0.36} & \textbf{96.98 $\pm$ 0.26} & \textbf{97.74 $\pm$ 0.27} \\
\hline
\citet{Straitouri2022ImprovingEP} official (single) & 98.98
$\pm$ 0.09 & 98.66
$\pm$ 0.10 & 98.87 $\pm$ 0.14 & 94.72 $\pm$ 0.36 & 97.84 $\pm$ 0.19     \\
\hline
    \end{tabular}
    % \vspace{5pt}
     \label{tab:cifar10h_results_baselines}
\end{table}



% Using m=5,10,15, show visualization for PreResNet and CNN
% How does our framework compare with the set predictor baselines? What can we observe from the results? Why is this the case?
\textbf{Comparison with Top-k Set Predictors.}
Figure \ref{fig:cifar10h_set_predictors_results} illustrates the empirical success probability on the test data for our conformal-based framework compared to the top-k set predictors. Our framework outperforms the top-k set predictors (with $k=4, 5, 6$) even though the average set size $\bar{k}$ is significantly lower. This empirical result underscores the general effectiveness of the conformal predictor, which proves advantageous in both single expert and multi-expert human-AI settings. 

\begin{figure}[ht!]
\centering
\begin{subfigure}{.495\textwidth}
  \centering
  \includegraphics[width=6.5cm]{images/topic_cifar/set_predictors/set_predictors_Preresnet_m=5.jpg}
  \caption{Using the pre-trained model Preresnet}
\end{subfigure}%
\begin{subfigure}{.495\textwidth}
  \centering
  \includegraphics[width=6.5cm]{images/topic_cifar/set_predictors/set_predictors_Densenet_m=5.jpg}
  \caption{Using the pre-trained model Densenet}
\end{subfigure}
\caption{Comparison of our conformal multi-expert approach to the top-k set predictor-based approach in both single expert and multi-expert settings. The average set size of the conformal-based approach using PreResNet is $\bar{k}=1.69$, whereas with DenseNet, it is $\bar{k}=1.42$.}
\label{fig:cifar10h_set_predictors_results}
\vspace{-1em}
\end{figure}




% How does the different frameworks compare to a single human expert? Why is this important? What are the advantages and disadvantages of each approach?
\textbf{Comparing Different Ways of Combining Expert Predictions and Conformal Sets.}
Figure \ref{fig:cifar10h_different_frameworks} illustrates that all conformal-based multi-expert approaches outperform the performance of a single human alone, showcasing the effectiveness of combination approaches within a conformal setting despite their simplicity. It is evident that the mode approach is the most effective during inference.
%Please refer to the Appendix for the case when $m=3$ and $m=10$.



\begin{figure}[t!]
\centering
\vspace{0.5em}
    \begin{subfigure}{.48\textwidth}
      \centering
      \includegraphics[width=7.2cm]{images/topic_cifar/topic_conformalized/conformalized_Densenet.jpg}
      % \caption{}
    \end{subfigure}%
\hfill 
    \begin{subfigure}{.48\textwidth}
      \centering
      \includegraphics[width=6.5cm]{images/topic_cifar/increasing_m/mult_expert_number_Preresnet.jpg}
      % \caption{}
      \label{fig:cifar10h_increasing_m_preresnet}
    \end{subfigure}
    \vspace{-1pt}
\caption{Left: Comparison of combination approaches in our conformal multi-expert framework using the pre-trained model DenseNet. Right: Visualization of the empirical success probability on the test data of our conformal multi-expert approach, experts team, and top-5 set predictor-based approach for varying numbers of multiple experts. The pre-trained model used is PreResNet.}
\vspace{-1.5em}
\label{fig:cifar10h_different_frameworks}
\end{figure}










% Plot for each of the pretrained model: densenet, resnet, preresnet, cnn, r_low_acc
% x-axis: values of m (1,2,3,4,5,6,7,8,9,10); y-axis: accuracy; plots of our multiple framework, top5 framework, mode policy AAMAS, expert team

% PUT IN CIFAR-10H
% Appendix for ImageNet-16H

% What is the observation? Does this make sense? Why is this the case?
\textbf{Comparison with Expert Team and top-5 set predictor-based approach with Varying Number of Experts on the Test Data}
In the right side of Figure \ref{fig:cifar10h_different_frameworks}, we compare the classification performance on the test set between the expert team and the top-5 set predictor for varying values of $m$. Algorithm \ref{algo:optimal_m}'s suggestion to use $\hat{m}=3$ for the PreResNet model is helpful in this case. Observably, with a high number of simulated human experts, the expert team outperforms both our conformal multi-expert approach and the top-5-based approach. This aligns with the intuition that a large number of human experts are capable of making accurate decisions. Figure \ref{fig:increasing_m_appendix} shows that with less accurate pre-trained models, our conformal multi-expert approach cannot outperform experts team for any number of human expert. On the other hand, in scenarios with one or a few multiple experts, leveraging conformal prediction to narrow down the sets to a subset benefits decision-making given that the pre-trained model is accurate. In practice, balancing the number of experts with available resources is crucial.


% We also observe that even with just the expert team, e.g. 30 experts, state-of-the-art performance on the ImageNet dataset can be achieved without the need for the model. And the AI model + many experts cannot outperform it. This is very problematic. %What is performance when the pretrained model is so good (better than human)? What is performance when the pretrained model is not that good (worse than human)?



















==> 4.old_experiments_imagenet.tex <==





















\subsubsection{ImageNet-16H Dataset}



% How does our framework compare with top-k predictors on the ImageNet-16H dataset? Why is this the case?
\textbf{Comparison with Top-k Predictors}. Table \ref{tab:set_baselines_results_imagenet} compares our conformal mode-based multi-expert approach against frameworks employing top-k set predictors. Our framework demonstrates superior empirical success probability, outperforming both single-expert and multi-expert baselines, even when the average set size $\bar{k}$ is smaller than $k$. This underscores the effectiveness of conformal prediction in facilitating effective Human-AI collaboration.



% PLOT/FIGURE Bar Plot vs Combine vs Singh vs EPCP vs Multi-expert EPCP
% 15-5-80
% Does increase in test make the accuracy increase? YES
% Appendix: show 3,7,10 experts
\textbf{Comparison with relevant human-AI baselines.}
Figure \ref{fig:baselines_imagenet} compares our framework to existing baselines. Our method outperforms the conformal set-based single human approach \citep{Straitouri2022ImprovingEP}. However, it achieves lower empirical success probability than the Mode approach \cite{Singh2023OnSS} due to limited calibration data and a higher number of classes compared to CIFAR-10H. Despite this, the conformal-based approach offers the advantage of providing fewer options for the human expert to choose from.
% We also note that we can further improve the performance of our approach by increasing the size of the calibration data.
% In Figure \ref{fig:cal_data_vs_succ}, we show the success probability of our approach compared to EPCP with varying percentage of the calibration data.



% 30-10-60//20-10-70//15-5-80
\begin{minipage}{0.55\textwidth}

    \centering
    \vspace{-1em}
    \begin{table}[H]
    \caption{Comparison of our conformal-based approach with top-k subset prediction frameworks on the ImageNet-16H dataset using two train-val-test splits, $v1$ and $v2$. For $v1$, average set size $\bar{k}=10.16$, while for $v2$, $\bar{k}=9.23$. Multi-expert teams comprise 5 experts.} 
    \vspace{1em}
    \setlength{\tabcolsep}{5.5pt}
        \centering
        \footnotesize 
        \begin{tabular}{|l|c|c|}
        \hline
            Methods &  $v1$ & $v2$           \\
            \hline
            Single Human	& 90.02 $\pm$ 0.93 &  90.05 $\pm$ 1.22   	                   \\ % 89.54 $\pm$ 1.67 &
            Model	    &	67.78 $\pm$ 1.33  &    70.90 $\pm$ 1.28                     \\  % 69.58 $\pm$ 1.23  &
            \hline 
            ⁠⁠Top-$k$ $(k=10)$ 	&	80.24 $\pm$ 1.91  &    80.00 $\pm$ 2.21     	    \\ % 76.17 $\pm$ 1.19 &
            Top-$k$ $(k=11)$	& 80.19 $\pm$ 1.96 &	  79.57 $\pm$ 2.09      	\\ % 76.27 $\pm$ 1.82  &
            Top-$k$ $(k=12)$	& 80.10 $\pm$ 2.19 &	  79.43 $\pm$ 1.95     	                   \\ % 76.79 $\pm$ 1.74  &
            \hline 
            Top-$k$ Multiple $(k=10)$	& 89.47 $\pm$ 1.54 &	  89.52 $\pm$ 1.36               \\ % 84.59 $\pm$ 1.02  &
            Top-$k$ Multiple $(k=11)$	& 89.52 $\pm$ 1.55 &	 90.00 $\pm$ 1.38                \\ % 85.50 $\pm$ 1.30  &
            Top-$k$ Multiple $(k=12)$	& 89.71 $\pm$ 1.37 &   90.00 $\pm$ 1.53             \\ % 86.51 $\pm$ 1.23	  &
            \hline 
            Conformal Single &	82.82 $\pm$ 0.99  &   80.68 $\pm$ 2.18                      \\ % 80.14 $\pm$ 1.90	&
            Conformal Multiple	 & \textbf{91.47 $\pm$ 0.65} &   \textbf{91.25 $\pm$ 1.05}                \\ % 91.16 $\pm$ 0.47 &
            \hline 
        \end{tabular}
        \vspace{5pt}
       
    \label{tab:set_baselines_results_imagenet}
    \end{table}
\end{minipage}%
\hspace{15pt}
\begin{minipage}{0.40\textwidth}
    \centering
    % 30-10-60//35-10-55//40-10-50
    % \vspace{-0.25em}
    \begin{figure}[H]
      \centering
      
      \includegraphics[width=5.25cm]{images/topic_imagenet/baselines.jpg}
      \caption{Comparison of our conformal multi-expert approach with Human-AI baselines on the Imagenet-16H dataset. }
      \vspace{30pt}
      \label{fig:baselines_imagenet}
    \end{figure}
    
\end{minipage}
% \vspace{-1em}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPENDIX
% INSERT GRAPH OF INCREASING m=1,2,3,4,5,6,7,8,9,10 (x-axis) of our Multiple vs topk k=10 multiple approaches (y-axis accuracies) vs Expert Team
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=9cm]{images/topic_imagenet/baselines.jpg}
%   \caption{Comparison of baselines.}
%   \label{fig:baselines_imagenet}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






% Unique to this dataset is the huge number of classes and limited calibration data
\textbf{Correlation of class-conditional coverage and the empirical success probability.} For a 16-class dataset with only 1200 samples split across training, validation, estimation, calibration, and testing, we observe a decline in class-specific coverage by the conformal prediction method due to limited calibration data (only less than 13 data points for each class). As illustrated in Figure \ref{fig:corr_cov_succ_imagenet}, this decrease in mean coverage adversely impacts the empirical success probability.
\vspace{-1em}













% \textbf{APPENDIX: RESULTS WITH DIFFERENT TYPES OF MULTIPLE EXPERT FUSION for ImageNet}
% \textbf{APPENDIX: SIZE DISTRIBUTION OF THE RECOMMENDED SUBSETS}
% \textbf{APPENDIX: PERFORMANCE UNDER DIFFERENT ALPHA VALUES}





\subsection{Limitations}
\label{limitations}
\vspace{-1em}


The conformal predictor relies on the calibration data to determine the threshold or quantile for the non-conformity scores \cite{Angelopoulos2023ConformalPA}. With few calibration samples, this threshold estimation can be inaccurate, leading to poor coverage guarantees. When most classes have very few calibration examples as in ImageNet-16H, this is not enough data to reliably estimate the class-conditional nonconformity score distributions needed for conformal prediction.
\vspace{-1em}
%Moreover, we empirically observe that the conformal-based multi-expert approach to outperform team of experts relies on the accuracy of the pre-trained model. 

% However, a potential limitation of our framework is the increased inference time due to the computation of individual expert predictions and the requirement for sufficient calibration data.
